Asymptotically Optimal Welfare of Posted Pricing for Multiple Items with MHR Distributions

We consider the problem of posting prices for unit-demand buyers if all $n$ buyers have identically distributed valuations drawn from a distribution with monotone hazard rate. We show that even with multiple items asymptotically optimal welfare can be guaranteed. Our main results apply to the case that either a buyer's value for different items are independent or that they are perfectly correlated. We give mechanisms using dynamic prices that obtain a $1 - \Theta \left( \frac{1}{\log n}\right)$-fraction of the optimal social welfare in expectation. Furthermore, we devise mechanisms that only use static item prices and are $1 - \Theta \left( \frac{\log\log\log n}{\log n}\right)$-competitive compared to the optimal social welfare. As we show, both guarantees are asymptotically optimal, even for a single item and exponential distributions.

==> alpha_correlation_matching.tex <==
\section{The case of correlation}
\label{section_alpha_correlation}

We start by considering correlated edge weights. Each offline node $j \in R$ has a deterministic node-specific multiplier $\alpha_j$ (which can be interpreted as a click through rate in online advertising \todo{For multiple items, we adopt the assumption of \emph{separable valuations}, which are common in ad auctions \citep{EdelmanOS07,Varian07}}), each online node $i \in L$ has a type $v_i$ drawn i.i.d from a distribution $\mathcal{D}$. The weight of edge $e = (i,j)$ is given by $v_{e} = \alpha_j \cdot v_i$. \\

The types $v_1, \ldots, v_n \geq 0$ are non-negative, independent and identically distributed random variables with a continuous distribution satisfying the MHR condition. Let $j_i \in R$ denote the offline node which is matched to node $i \in L$ in our algorithm and set $j_i = m+1$ with $\alpha_{m+1} = 0$ if $i$ is not matched at all. We can specify the expected weight of the matching of the algorithm as $\Ex[]{\sum_{i = 1}^n \alpha_{j_i} v_i }=: \Ex[]{\ALG}$. \\

Without loss of generality, we assume that $\alpha_1 \geq \alpha_2 \geq \ldots$ and that $m = n$. The former can be ensured by reordering the nodes in $R$; the latter by adding nodes in $R$ with $\alpha_j = 0$ or removing all nodes $j \in R$ with $j > n$ respectively. Note that this setup also contains the typical i.i.d. prophet inequality scenario where we can select one of $n$ values: To derive this, set $\alpha_1 = 1, \alpha_2 = \ldots = 0$. Even further, the $k$-select i.i.d. prophet problem can be modeled by $\alpha_1 = \ldots = \alpha_k = 1, \alpha_{k+1} = \ldots = 0$. \\

Using the structure of correlated weights, the structure of the optimal matching can be stated in a more detailed way. Given any type profile $\mathbf{v} = (v_1, \ldots, v_n)$, let $v_{(k)}$ denote the $k$-th highest order statistics. That is $v_{(k)}$ is the largest $x$ such that there are at least $k$ entries in $\mathbf{v}$ whose value is at least $x$. Denote its expectation by $\Ex[]{v_{(k)}} = \mu_k$. The maximum-weight matching assigns offline node $1$ to an online node of type $v_{(1)}$, offline node $2$ to an online node of type $v_{(2)}$ and so on. Hence, the expected maximum-weight matching is given by $\Ex[]{\OPT} = \Ex{\sum_{j = 1}^m \alpha_j v_{(j)}} = \sum_{j = 1}^m \alpha_j \mu_j$. \\

We construct two threshold-based algorithms. The first using dynamic thresholds which can be adapted with respect to previously chosen edges, the second one using static thresholds which have to be determined a priori.  



%Instead of having independent item valuations, we consider the case of correlated ones. Our results concern a single and multiple items. For multiple items, we adopt the assumption of \emph{separable valuations}, which are common in ad auctions \citep{EdelmanOS07,Varian07}. Again, we restrict to the class of unit-demand buyers. In order to determine buyer $i$'s value for item $j$, let each buyer $i$ have a type $v_i \geq 0$ (here, $v_i$ is not a function but a random variable) and let each item have an item-dependent multiplier $\alpha_j$ which can be interpreted as a click through rate in online advertising. Buyer $i$'s valuation function $v_i (\{j\})$ for being assigned item $j$ simplifies to $\alpha_j \cdot v_i$. Without loss of generality, we assume that $\alpha_1 \geq \alpha_2 \geq \ldots$ and that $m = n$. The former can be ensured by reordering the items; the latter by adding items with $\alpha_j = 0$. Note that this correlation setup also contains the single-item scenario as a special case since it can be modeled by $\alpha_1 = 1, \alpha_2 = \ldots = 0$. More generally, $k$ identical items can be modeled by $\alpha_1 = \ldots = \alpha_k = 1, \alpha_{k+1} = \ldots = 0$. 

%The types $v_1, \ldots, v_n \geq 0$ are non-negative, independent identically distributed random variables with a continuous distribution satisfying the MHR condition. Let $j_i$ denote the item allocated to buyer $i$ and $j_i = m+1$ if buyer $i$ is not allocated any item where $\alpha_{m+1} = 0$. We can specify the expected social welfare of the mechanism as $\Ex[]{\sum_{i = 1}^n \alpha_{j_i} v_i }=: \Ex[]{\ALG}$.

%Additionally, the structure of the optimal allocation can be stated in a more detailed way. Given any type profile $v = (v_1, \ldots, v_n)$, we let $v_{(k)}$ denote the $k$-th highest order statistics. That is $v_{(k)}$ is the largest $x$ such that there are at least $k$ entries in $v$ whose value is at least $x$. Denote its expectation by $\Ex[]{v_{(k)}} = \mu_k$. The allocation that maximizes social welfare assigns item $1$ to a buyer of type $v_{(1)}$, item $2$ to a buyer of type $v_{(2)}$ and so on. Hence, the expected optimal social welfare is given by $\Ex[]{\OPT} = \Ex{\sum_{j = 1}^m \alpha_j v_{(j)}} = \sum_{j = 1}^m \alpha_j \mu_j$.


\subsection{Dynamic Threshold Algorithm}
\label{section:alpha_correlation_dynamic}

Our dynamic threshold algorithm is stated in Algorithm \ref{algorithm_dynamic_correlated}. \todo{Evtl sollten wir diesen Algorithmus auch als generelles Framework vorziehen, und dann jeweils nur die spezifischen Algorithmen darstellen??}

\begin{algorithm}[h]
	\SetAlgoNoLine
	\DontPrintSemicolon
	%\KwData{Sellers, indexed $1,\dots,m$ and buyers, indexed $m+1, \dots m+n$}
%	\KwResult{Set $A = A_B \cup A_S$ of agents to get an item with $A_B \subseteq B$, $A_B \in \mathcal{I}_B$, $A_S \subseteq S$ and $|A| = |S|$}
%	$A \longleftarrow \emptyset$ ; \qquad $A' \longleftarrow \emptyset$ ; \qquad  $M_{\textnormal{SELL}} \longleftarrow \emptyset$; \qquad $T = \left( 0, \dots, 0 \right)$, where $T$ is a vector of zeros of size $|S|$ \\
	$R^{(1)} \longleftarrow R$ \\
	\For{$i \in L$}{
		\text{Recompute $p_j^{(i)}$ for any $j \in R^{(i)}$} \\
		\text{Set $j_i \in \arg\max_{j \in R^{(i)}} \{ v_{ij} - p_j^{(i)} \}$ and remove $j_i$ from $R^{(i+1)}$ } 
	}
	\caption{Dynamic Threshold Algorithm}
	\label{algorithm_dynamic_correlated}
\end{algorithm}

Consider step $i$ and node $i$ arrives. Let $R^{(i)}$ be the set of unmatched offline at this time. We set thresholds to ensure that every node is matched and no online node remains unmatched. Therefore, always $\lvert R^{(i)} \rvert = n - i + 1$.

We choose thresholds $(p^{(i)}_j)_{j \in R^{(i)}}$ with the goal that we pick each edge with probability $\frac{1}{n - i + 1}$. To this end, \todo{Change notation from ell to something more like r} let $R^{(i)} = \{ \ell_1, \ldots, \ell_{n-i+1} \}$ with $\ell_1 < \ell_2 < \ldots < \ell_{n-i+1}$ and set
\[
p_j^{(i)} = \sum_{k: j \leq \ell_k \leq n-i} (\alpha_{\ell_k} - \alpha_{\ell_{k+1}}) F^{-1}\left( 1 - \frac{k}{n - i + 1}\right) \enspace.
\]
In principle, the weight of two edges $(i,j)$ and $(i,j')$ is the same if $\alpha_j = \alpha_{j'}$. As we define new thresholds in the next iteration anyway, we can assume that ties are broken in our favor. That is why we will assume in the following that online node $i$ is matched to $\ell_k$ if and only if $F^{-1}\left( 1 - \frac{k}{n - i + 1}\right) \leq v_i < F^{-1}\left( 1 - \frac{k-1}{n - i + 1}\right)$. 

%\begin{restatable}{theorem}{alphacorrelationdynamic}
\begin{theorem}
	\label{theorem:alpha_correlation_dynamic-positive}
	%The posted-prices mechanism with dynamic prices, unit-demand buyers and alpha-correlated valuations is $1 - O\left( \frac{1}{\log n} \right)$-competitive with respect to social welfare.
	The dynamic threshold algorithm for alpha-correlated edge weights is $1 - O\left( \frac{1}{\log n} \right)$-competitive.
\end{theorem}
%\end{restatable}


\todo{Maybe use this representation of the algorithm:}


\begin{algorithm}[h]
	\SetAlgoNoLine
	\DontPrintSemicolon
	%\KwData{Sellers, indexed $1,\dots,m$ and buyers, indexed $m+1, \dots m+n$}
	%	\KwResult{Set $A = A_B \cup A_S$ of agents to get an item with $A_B \subseteq B$, $A_B \in \mathcal{I}_B$, $A_S \subseteq S$ and $|A| = |S|$}
	%	$A \longleftarrow \emptyset$ ; \qquad $A' \longleftarrow \emptyset$ ; \qquad  $M_{\textnormal{SELL}} \longleftarrow \emptyset$; \qquad $T = \left( 0, \dots, 0 \right)$, where $T$ is a vector of zeros of size $|S|$ \\
	$R^{(1)} \longleftarrow R$ \\
	\For{$i \in L$}{
		\text{Let $k$ be such that $F^{-1}\left( 1 - \frac{k}{n - i + 1}\right) \leq v_i < F^{-1}\left( 1 - \frac{k-1}{n - i + 1}\right)$} \\
		\text{Set $j_i = \ell_k$ and remove $j_i$ from $R^{(i+1)}$ } 
	}
	\caption{Dynamic Threshold Algorithm}
	\label{algorithm_dynamic_correlated_2}
\end{algorithm}






\todo{until here}
We defer the proof to Appendix~\ref{appendix:correlated_valuations}. The main ideas are similar to the proofs of competitive ratios for the case of dynamic prices in the previous sections. In contrast, due to the specific structure of the valuations, we can now give a lower bound for buyer $i$'s value if buyer $i$ prefers item $j$. From the technical point of view, we apply the lemma from the static-pricing case and additionally introduce another lemma to bound the $(1-q)$-quantile of any MHR distribution with the expectation of the $\left\lfloor nq + \sqrt{n \log n} \right\rfloor$-th order statistic.  \\

Again by Section \ref{section:optimality}, this competitive ratio is optimal.






\subsection{Static prices}
\label{section:alpha_correlation_static}
We start with the case of static prices. Therefore, we define probabilities $q_j$ having the interpretation that a buyer drawn from the distribution has one of items $1, \ldots, j$ as their first choice. For technical reasons, we discard items $m + 1, \ldots, n$ for $m = n - n^{5/6}$ by setting $p_j = \infty$ for these items. For $j \leq m$, we set prices
\[
p_j = \sum_{k = j}^n (\alpha'_k - \alpha'_{k+1}) F^{-1}(1 - q_k) \enspace, \text{ where } q_k = \min\left\{ \frac{k}{n} 2 \log \log n, \frac{k}{n} + \sqrt{\frac{\log n}{n}} \right\} \enspace,
\]
where $\alpha'_k = \alpha_k$ for $k \leq m$ and $0$ otherwise. 

Note the similarity of this price definition to the payments when applying the VCG mechanism. There, the buyer being assigned item $j$ has to pay $\sum_{k = j}^n (\alpha'_k - \alpha'_{k+1}) v_{(k + 1)}$.


%\begin{restatable}{theorem}{alphacorrelationstaticpositive}
\begin{theorem}
	\label{theorem:alpha_correlation_staticpositive}
	The static-price mechanism with unit-demand buyers and alpha-correlated valuations is $1 - O\left(\frac{\log \log \log n}{\log n}\right)$-competitive with respect to social welfare.
\end{theorem}
%\end{restatable}

The proof of this theorem is deferred to Appendix~\ref{appendix:correlated_valuations} and quickly sketched here. We begin by showing a lemma which says that the prices are low enough so that we can guarantee to allocate all items with a reasonably high probability of at least $1 - \frac{111}{\log n}$. Next, we derive a generalized version of Lemma \ref{lemma:lower_bound_on_cdf_with_max} in order to bound the quantiles of any MHR distribution from below by the expectation of any order statistic. Having this, we decompose the social welfare into utility and revenue. The revenue of our mechanism is bounded in terms of the VCG revenue by an application of the two lemmas. Talking about utility, we use a link to Myerson's theory and virtual values in order to achieve our desired bound. \\ 

As before, also our optimality results from Section \ref{section:optimality} apply.


==> dynamic.tex <==
% !TEX root = mhr-prophet.tex
\section{Dynamic Pricing}
\label{section:dynamic}
In this section, we give a posted-prices mechanism with an improved competitive ratio by using dynamic prices. That is, the prices offered to buyer $i$ depend on which items are still available.

In step $i$, buyer $i$ arrives. Let $M^{(i)}$ be the set of remaining items at this time. Our choice of prices ensures that in each step one item is allocated. Therefore, always $\lvert M^{(i)} \rvert = n - i + 1$.

We choose prices $(p^{(i)}_j)_{j \in M^{(i)}}$ with the goal that each item is allocated with probability $\frac{1}{n - i + 1}$. To this end, let $M^{(i)} = \{ \ell_1, \ldots, \ell_{n-i+1} \}$ with $\ell_1 < \ell_2 < \ldots \leq \ell_{n-i+1}$ and set
\[
p_j^{(i)} = \sum_{k: j \leq \ell_k \leq n-i} (\alpha_{\ell_k} - \alpha_{\ell_{k+1}}) F^{-1}\left( 1 - \frac{k}{n - i + 1}\right) \enspace.
\]
In principle, buyers will be indifferent between two items $j$ and $j'$ if $\alpha_j = \alpha_{j'}$. As these items are indistinguishable for later buyers anyway and new prices will be defined, we can assume that ties are broken in our favor. That is why, we will assume in the following that a buyer $i$ will prefer item $\ell_k$ if and only if $F^{-1}\left( 1 - \frac{k}{n - i + 1}\right) \leq v_i < F^{-1}\left( 1 - \frac{k-1}{n - i + 1}\right)$. \later{This argument could be better.}

\begin{theorem}
\label{theorem:dynamic-positive}
The posted-prices mechanism with dynamic prices is $1 - O\left( \frac{1}{\log n} \right)$-competitive.
\end{theorem}

To prove this theorem, we will need another bound relating quantiles to expected order statistics, in the spirit of Lemma~\ref{lemma:quantiles1}.

\begin{lemma}
\label{lemma:quantiles2}
For all $q \in [0, 1]$, we have
\[
F^{-1}(1 - q) \geq \mu_{\left\lfloor nq + \sqrt{n \ln n} \right\rfloor} \enspace.
\]
\end{lemma}

\begin{proof}
Let $y = F^{-1}(1 - q)$ and $k = \left\lfloor nq + \sqrt{n \ln n} \right\rfloor$\later{integrality}. Define independent Bernoulli random variables $Z_i$ by setting $Z_i = 1$ if $v_i \geq y$ and $0$ otherwise. By this definition, $\Ex{Z_i} = q$. Furthermore, define $Z = \sum_{i = 1}^n Z_i$. Observe that $v_{(k)} < y$ if and only if $\sum_{i = 1}^n Z_i < k$.

By Hoeffding's inequality, using $\Ex{Z} = n q$, we have
\[
\Pr{Z \geq k} = \Pr{Z \geq nq + \sqrt{n \ln n}} \leq \exp\left( - 2 \frac{n \ln n}{n} \right) = \frac{1}{n^2} \enspace.
\]
And therefore
\[
\Pr{v_{(k)} < y} = \Pr{Z < k} \geq 1 - \frac{1}{n^2} \enspace.
\]
%\begin{lemma}[\cite{rinne2014hazard}]
%	\label{lemma:mhr_property_of_order_statistics}
%	For any continuous \textnormal{MHR} random variable $X$ and integers $1 \leq k \leq n$, the $k$-th lowest order statistic $X_{k:n}$ out of $n$ i.i.d. draws is also distributed according to an MHR distribution.
%\end{lemma}
%
%\begin{lemma}[cf. \cite{barlow1964}, Theorem 3.8]
%	\label{lemma:mhr_properties}
%	Let $X$ be a continuous MHR random variable with CDF $F$ and known expectation $\mu := \Ex{X}$. Then, a sharp lower bound for $1-F(x)$ is
%	\begin{equation*}
%	1 - F(x) \geq 
%	\begin{cases}
%	e^{-\frac{x}{\mu}} & \;,\; x \leq \mu \\
%	0 & \;,\; x > \mu
%	\end{cases}
%	\end{equation*}
%\end{lemma}
\later{Re-insert lemma statements?}
Furthermore, as $v_{(k)}$ is an order statistic, it is distributed according to an MHR distribution \cite{rinne2014hazard}. Therefore (cf. \cite{barlow1964}, Theorem 3.8)
\[
\Pr{v_{(k)} \leq \mu_k} \leq 1 - \frac{1}{e} \enspace.
\]
Therefore, since $n^2 \geq e$, we have to have $\mu_k \leq y$.
\end{proof}

Now, we are ready to prove the theorem.

\begin{proof}[Proof of Theorem~\ref{theorem:dynamic-positive}]
For any buyer $i$ and available item $j \in M^{(i)}$, let $w^{(i)}_j$ be smallest type for buyer $i$ such that item $j$ is the preferred one. Furthermore, let $X_{i, j} = 1$ if item $j$ gets allocated in step $i$.

Observe that the social welfare of the final allocation is at least
\[
\sum_{i = 1}^n \sum_{j = 1}^n \alpha_j w^{(i)}_j X_{i, j} \enspace.
\]
Furthermore, by our construction
\[
\Pr{X_{i, j} = 1} = \frac{1}{n - i + 1} \prod_{i' = 1}^{i-1} \left( 1 - \frac{1}{n - i' + 1} \right) = \frac{1}{n} \enspace.
\]
Note that also $w^{(i)}_j$ is a random variable and our goal will be to lower-bound its expectation. Let $Z = j - 1 - \sum_{i' = 1}^{i - 1} \sum_{j' = 1}^{j - 1} X_{i', j'}$ be a random variable indicating the number of items of smaller index that are included in $M^{(i)}$. By this definition $w^{(i)}_j = F^{-1}\left( 1 - \frac{Z + 1}{n - i + 1} \right)$.

%For $j \leq n^{\frac{2}{3}}$, set $c = \frac{\ln(n - i + 1) - \ln j}{H_n - H_{j-1}}$ and apply Lemma~\ref{lemma:mhrorderstatistics}. It implies
%\[
%\Pr{v_t \geq c \Ex{v_{(j)}}} \geq \exp\left( -c (H_n - H_{j-1}) \right) = \frac{j}{n - i + 1} \enspace.
%\]
%Note that $\Pr{v_t \geq w^{(i)}_j} \leq \frac{j}{n - i + 1}$, so
We distinguish two cases. First, consider $j \leq n^{2/3}$. We use that $Z + 1 \leq j$. Therefore, by Lemma~\ref{lemma:quantiles1}, we have
\[
w^{(i)}_j = F^{-1}\left( 1 - \frac{Z + 1}{n - i + 1} \right) \geq F^{-1}\left( 1 - \frac{j}{n - i + 1} \right) \geq  \frac{\ln(n - i + 1) - \ln j}{H_n - H_{j-1}} \mu_j \enspace.
\]
Observe that this lower bound is not a random variable. Therefore, we can write
\[
\Ex{\sum_{i = 1}^n w^{(i)}_j X_{i, j}} \geq \sum_{i = 1}^n \frac{\ln(n - i + 1) - \ln j}{H_n - H_{j-1}} \mu_j \Ex{X_{i, j}} \enspace.
\]
By applying the integral estimation $\sum_{i = 1}^n \ln(n - i + 1) \geq n \ln n - n + 1$ and using that $\Ex{X_{i, j}} = \frac{1}{n}$, this term is at least
\[
\frac{\ln n - 1 + \frac{1}{n} - \ln j}{H_n - H_{j-1}} \mu_j \geq \frac{\ln n - \ln j - 1}{\ln n - \ln j + 2} \mu_j = \left( 1 - \frac{3}{\ln n - \ln j + 2} \right) \mu_j \geq \left( 1 - \frac{9}{\ln n} \right) \mu_j \enspace.
\]

For $j > n^{\frac{2}{3}}$, we only consider $i \leq \left( 1 - \frac{1}{\ln n} \right) n$. Note that $Z$ is essentially the outcome of sampling without replacement. Conditional on $j \in M^{(i)}$, we have
\[
\Pr{j' \in M^{(i)} \growingmid j \in M^{(i)}} = \frac{n - i}{n - 1}
\]
and so
\[
\Ex{Z \growingmid j \in M^{(i)}} = (j-1) \frac{n - i}{n - 1} \enspace.
\]
We can apply Hoeffding's inequality and get
\[
\Pr{Z \leq (j-1) \frac{n - i}{n - 1} - \sqrt{n \ln n} \growingmid j \in M^{(i)}} \leq \exp\left( - 2 \frac{n \ln n}{i - 1} \right) \leq \frac{1}{n^2} \enspace.
\]

Observe that $(j - 1)(n - i) + (n - 1) \geq j (n - i + 1) - n$ so, if $Z > (j-1) \frac{n - i}{n - 1} - \sqrt{n \ln n}$, then also $Z + 1 > \frac{j}{n-1}(n - i + 1) - \frac{n}{n-1} - \sqrt{n \ln n}$. Therefore, if $i \leq \left( 1 - \frac{1}{\ln n} \right) n$
\[
\Pr{\frac{Z + 1}{n - i + 1} > \frac{j}{n} - \frac{2 (\ln n)^{3/2}}{\sqrt{n}} \growingmid j \in M^{(i)}} \geq \Pr{\frac{Z + 1}{n - i + 1} > \frac{j}{n} - \frac{2 + \sqrt{n \ln n}}{n - i + 1} \growingmid j \in M^{(i)}} \geq 1 - \frac{1}{n^2} \enspace.
\]
So, by Lemma~\ref{lemma:quantiles2}, we get that
\[
\Pr{w^{(i)}_j > \mu_{\lfloor j + \sqrt{n \ln n} + 2 \sqrt{n} (\ln n)^{3/2} \rfloor}  \growingmid j \in M^{(i)}} \geq 1 - \frac{1}{n^2} \enspace.
\]
Consequently, \later{Use Union Bound argument instead.}
\[
\Ex{w^{(i)}_j X_{i, j}} \geq \left( 1 - \frac{1}{n^2} \right) \cdot \mu_{\lfloor j + \sqrt{n \ln n} + 2 \sqrt{n} (\ln n)^{3/2} \rfloor} \Ex{X_{i, j}} \enspace.
\]
Therefore, we get
\[
\Ex{\sum_{i = 1}^n w^{(i)}_j X_{i, j}} \geq \Ex{\sum_{i = 1}^{(1 - \frac{1}{\ln n})n} w^{(i)}_j X_{i, j}} \geq \left(1 - \frac{1}{\ln n} \right) \mu_{\lfloor j + \sqrt{n \ln n} + 2 \sqrt{n} (\ln n)^{3/2} \rfloor} \enspace.
\]

Combining these bounds for all $j$, we get
\begin{align*}
\Ex{\sum_{i = 1}^n \sum_{j = 1}^m \alpha_j w^{(i)}_j X_{i, j}} & = \sum_{j = 1}^{\lfloor n^{2/3} \rfloor} \Ex{\sum_{i = 1}^n \alpha_j w^{(i)}_j X_{i, j}} + \sum_{j = \lfloor n^{2/3} \rfloor + 1}^{n} \Ex{\sum_{i = 1}^n \alpha_j w^{(i)}_j X_{i, j}} \\
& \geq \left(1 - \frac{9}{\ln n} \right) \sum_{j = 1}^{\lfloor n^{2/3} \rfloor} \alpha_j \mu_j + \left( 1 - \frac{1}{\ln n} \right) \sum_{j = \lfloor n^{2/3} \rfloor + \lfloor \sqrt{n \ln n} + 2 \sqrt{n} (\ln n)^{3/2} \rfloor + 1}^{n} \alpha_j \mu_j \\
& \geq \left( 1 - O\left( \frac{1}{\ln n} \right) \right) \sum_{j = 1}^m \alpha_j \mu_j \enspace. \qedhere
\end{align*}
\end{proof}

\subsection{Optimality}
We will now show that the guarantee of our dynamic-pricing mechanism is also optimal. Even with a single item and types drawn from an exponential distribution, the best competitive ratio is $1 - \Omega\left(\frac{1}{\ln n}\right)$.

\begin{proposition}
	\label{proposition:optimality-dynamic}
	Let $v_1, \dots, v_n \in \mathbb{R}_{\geq 0}$ be random variables where each $v_i$ is drawn i.i.d. from the exponential distribution with rate $1$, i.e., $v_1, \ldots, v_n \sim \mathrm{Exp}(1)$. For all dynamic prices, the competitive ratio of the mechanism picking the first $v_i$ with $v_i \geq p^{(i)}$ is upper bounded by $1 - \Omega\left(\frac{1}{\ln n}\right)$.
\end{proposition}

We will use that the expected value of the optimal offline solution (the best value in hindsight) is given by $\Ex[]{\max_i v_i} = H_n$ \cite{Arnold:2008:FCO:1373327}. Therefore, it suffices to show that the expected value of any dynamic prices is upper bounded by $H_n - c$ for some constant $c > 0$.

To upper-bound the expected social welfare of any dynamic pricing, we use the fact that this problem corresponds to a Markov decision process and the optimal dynamic prices are given by\footnote{To the best of our knowledge, this is a folklore result.}
\[
p^{(n)} = 0 \quad \text{ and } \quad p^{(i)} = \Ex[]{\max \{v_{i+1}, p^{(i+1)}\}} \quad \text{ for $i < n$} \enspace.
\]
Furthermore, $p^{(0)}$ is exactly the expected social welfare of this mechanism. Therefore, the following lemma with $k = n$ directly proves our claim.

\begin{lemma}
	\label{lemma:mdp-recursion}
	Let $v_1, \dots, v_n \in \mathbb{R}_{\geq 0}$ be random variables where each $v_i$ is drawn i.i.d. from the exponential distribution $\textnormal{Exp}(1)$. Moreover, let $p^{(n)} = 0$ and $p^{(i)} = \Ex[]{\max \{v_{i+1}, p^{(i+1)}\}}$ for $i < n$. Then, we have $p^{(n-k)} \leq H_k - \frac{1}{8}$ for all $2 \leq k \leq n$.
\end{lemma}
	
\begin{proof}
	We are going to prove the statement by induction on index variable $k$.\\
	
	First, consider the induction base $k = 2$. By definition of the thresholds we know that $p^{(n)} = 0$ and $p^{(n-1)} = \Ex{\max \{v_n, p^{(n)} \}} = \Ex{\max \{v_n, 0 \}} = \Ex{v_n} = 1$. Next, consider the threshold $p^{(n-2)}$ defined by
	\begin{align*}
	p^{(n-2)} &= \Ex{\max \{v_{n-1}, p^{(n-1)} \}} = \Ex{\max \{v_{n-1}, 1 \}} \\
	&= \int_{0}^{\infty} \Pr{\max\{v_{n-1}, 1\} \geq x} \mathrm{d}x = \int_{0}^{1} 1 \mathrm{d}x + \int_{1}^{\infty} e^{-x} \mathrm{d}x = 1 + \frac{1}{e} \approx 1.368 \,.
	\end{align*}
	Thus, we can easily verify that $p^{(n-2)} \leq 1.375 = H_2 - \frac{1}{8}$.\\
	
	For the inductive step, we move from $k$ to $k+1$. By the induction hypothesis, we have
	\[
	p^{(n-(k+1))} = \Ex{\max \{v_{n-k}, p^{(n-k)} \}} \leq \Ex{\max \left\{v_{n-k}, H_k - \frac{1}{8} \right\}} \enspace.
	\]
	Furthermore
	\begin{align*}
	\Ex{\max \left\{v_{n-k}, H_k - \frac{1}{8} \right\}} & = \int_{0}^{\infty} \Pr{\max\left\{v_{n-k}, H_k - \frac{1}{8}\right\} \geq x} \mathrm{d}x = \int_{0}^{H_k - \frac{1}{8}} 1 \mathrm{d}x + \int_{H_k - \frac{1}{8}}^{\infty} e^{-x} \mathrm{d}x \\
	& = H_k - \frac{1}{8} + e^{-H_k + \frac{1}{8}} \enspace.
	\end{align*}
	We now use the fact that the $k$-th harmonic number $H_k$ for $k \geq 2$ is bounded from below by $H_k \geq \ln k + \gamma$, in which $\gamma \approx 0.577$ denotes the Euler-Mascheroni constant. So for $k \geq 2$
	\[
	e^{-H_k + \frac{1}{8}} \leq e^{-(\ln k + \gamma) + \frac{1}{8}} = \frac{e^{\frac{1}{8} - \gamma}}{k} \leq \frac{e^{\frac{1}{8} - 0.57}}{k} \leq \frac{1}{\frac{3}{2} \cdot k} \leq \frac{1}{k+1} \enspace.
	\]
	In combination, this gives us
	\[
	p^{(n-(k+1))} \leq H_k - \frac{1}{8} + \frac{1}{k+1} = H_{k+1} - \frac{1}{8} \enspace.
	\]
\end{proof}

==> mhr_marginals.tex <==
% !TEX root = mhr-prophet.tex
\section{Arbitrary subadditive valuations with MHR marginals}
\label{section:mhr_marginals}
%In this section, we show our first set of results, which hold in very general settings. We can achieve asymptotically optimal bounds on the expected welfare and revenue by only assuming subadditive buyers as well as MHR distributions on the valuations for single items $v_i(\{j\})$.

In order to familiarize with the topic, we show our first set of results which hold in very general settings. We can achieve asymptotically optimal bounds on the expected welfare and revenue by only assuming subadditive buyers as well as MHR distributions on the valuations for single items $v_i(\{j\})$. This way, we naturally extend the well-known MHR definition for the value of a single item to the case of multiple heterogeneous items with possible correlations among them, as already discussed in Section \ref{section:introduction}. Note that subadditive valuation functions cover a lot of common cases, such as unit-demand, additive, XOS or submodular. We are able to show bounds on the welfare and revenue which match the upper bound results from Section \ref{section:optimality} when restricting to a single item. The strength of the results by our weak assumptions is at the expense of the fact that the bounds only give asymptotically full efficiency if the number of items satisfies $m = n^{o(1)}$. In order to improve these results, we show in Sections \ref{section:independent_valuations} and \ref{section_alpha_correlation} how to overcome this weakness using additional assumptions. 

\subsection{Static Prices}
\label{section:mhr_marginals_static}
We start by examining the case of static prices. That is, the price for an item remains unchanged while it is not sold, regardless of how much time has passed or which other items might have been sold. Our first result is a $1 - O \left( \frac{\log\log\log n}{\log n} + \frac{\log m}{\log n}\right)$-competitive static-price mechanism. 

The general design idea for our mechanism is as follows. Setting fairly low prices will put high probability on the event of selling all items. Although we cannot control which buyer will buy which bundle of items, we can extract all social welfare of the posted prices mechanism as revenue. Therefore, having prices which still ensure that the revenue can be lower bounded by a suitable fraction of the optimal social welfare will lead to the desired bound.


% Given any static prices $p_1, \ldots, p_m$, we can consider the probability that a random buyer drawn from the distribution prefers a fixed item. It seems reasonable to adjust prices so that this probability is $\frac{1}{n}$ for every item. This choice would ensure that in expectation one buyer from the sequence will have the item as her first choice. However, in the single-item setting, setting the probability to $\frac{1}{n}$ will cause the item to remain unsold with constant probability and thus we would get only a constant-factor approximation to the optimal social welfare. In the multi-item setting, there can also be two or more buyers be interested in the same bundle of items. This has the difficult consequence that when a specific bundle is sold, buyers will switch to other ones instead. That is, the probability of a bundle being the preferred one increases over time as a consequence of a non-trivial stochastic process. Gaining control over this selling-process is extremely difficult. Luckily, we are able to bound the effects in our argument. \todo{Edit}

For any item, we set the price of item $j$ to \[ p_j = F_j^{-1} \left( 1 - q \right) \textnormal{, where } q = \frac{m \log \log n}{n}  \] and $F_j$ denotes the marginal distribution of $v_i(\{j\})$. This allows us to prove the following theorem. 


\begin{restatable}{theorem}{staticmhrmarginals}
	\label{theorem:static_mhr_marginals}
	The posted-prices mechanism with subadditive buyers and static prices is \newline $1 - O \left( \frac{\log\log\log n}{\log n} + \frac{\log m}{\log n}\right)$-competitive with respect to social welfare. 
\end{restatable}

Especially worth mentioning, this ensures asymptotically full efficiency as the number of buyers becomes large compared to the number of items. Before proving the theorem, we start by a lemma concerning MHR distributions. By $H_n$ we denote the $n$-th harmonic number.

\begin{lemma}
	\label{lemma:lower_bound_on_cdf_with_max}
	\todo{remove this lemma completely!}For $i=1,\dots,n$, let $X_i$ be an i.i.d. draw from a non-negative MHR distribution with CDF $F$ and PDF $f$. For any real $q \in [\exp(-H_n),1]$, we have
	\begin{equation*}
		F^{-1}(1-q) \geq - \frac{\log q}{H_n} \Ex[]{\max_{i \in [n]} X_i } \ .
	\end{equation*}
\end{lemma}

\begin{proof}
	Let $X := \max_{i \in [n]} X_i$ with $\mu = \Ex[]{X}$. By the MHR property, $\log \left(
	 1 - F(\cdot) \right)$ is concave. Together with Jensen's inequality, we get 
	 \begin{align*}
	 	\log \left(1 - F\left( - \frac{\log q}{H_n} \mu \right) \right) & \geq - \frac{\log q}{H_n} \log \left(1 - F\left( \mu \right) \right) \geq - \frac{\log q}{H_n} \Ex[]{\log \left(1 - F\left( X \right) \right)}
	 \end{align*}
	 In order to compute the last expectation, we apply two changes of variables $u = F(y)$ and $t = - \log(1-u)$. 
	 \begin{align*}
		 \Ex[]{\log \left(1 - F\left( X \right) \right)} & =  \int_{0}^{\infty} \log(1-F(y)) n F^{n-1}(y) f(y) dy = \int_{0}^{1} \log(1-u) n u^{n-1} du \\ & = - \int_{0}^{\infty} t n \left( 1 - e^{-t} \right)^{n-1} e^{-t} dt = - \Ex[]{\max_{i \in [n]} Y_i}
	 \end{align*}
	 By $Y_i \sim \mathrm{Exp}(1)$ we denote i.i.d. exponential random variables, hence by \cite{Arnold:2008:FCO:1373327}, we have that $\Ex{\max_{i \in [n]} Y_i} = H_n$. Plugging these together, taking the exponential on both sides and rearranging terms proves the claim. %leads to 
	% \[ 1 - F\left( - \frac{\log q}{H_n} \mu \right) \geq q \] or equivalently \[ F^{-1} (1-q) \geq - \frac{\log q}{H_n}  \Ex[]{\max_{i \in [n]} X_i } \ . \]
\end{proof}

Now, we are ready to prove Theorem~\ref{theorem:static_mhr_marginals}.

\begin{proof}[Proof of Theorem~\ref{theorem:static_mhr_marginals}] 
	Lower bounding the expected revenue by a suitable fraction of the optimal social welfare will allow to prove the theorem.
	
	Recall that by our assumption $v_i(\{j\})$ is an MHR random variable for each $j \in [m]$. Therefore, we can apply Lemma~\ref{lemma:lower_bound_on_cdf_with_max} to get a bound on $p_j$.
	\begin{align*}
		p_j & = F_j^{-1} \left(1-q\right) \geq \frac{- \log q}{H_n} \Ex[]{\max_{i \in [n]} v_i(\{j\})} = \frac{\log n - \log \log \log n - \log m}{H_n} \Ex[]{\max_{i \in [n]} v_i(\{j\})} \\ & \geq \left( 1 - \frac{\log \log \log n + \log m + 1}{\log n} \right) \Ex[]{\max_{i \in [n]} v_i(\{j\})} .
	\end{align*} \newline
	
	Now, we aim for a lower bound on the probability that all items are sold in our mechanism. To this end, let $M^{(i)}$ denote the (random) set of items that are still unsold as buyer $i$ arrives. Observe that buyer $i$ will buy at least one item if $v_i(\{j\}) > p_j$ for some $j \in M^{(i)}$. We defined the prices such that $\Pr{v_i(\{j\}) > p_j} = q$. Consequently, $\Pr{\text{buyer $i$ buys an item} \growingmid M^{(i)} \neq \emptyset} \geq q$ for all $i$.
	
	To bound the probability of selling all items, consider the following thought experiment: For every buyer $i$, we toss a coin which shows head with probability $q$. Denote by $Z$ the random variable counting the number of occurring heads in $n$ coin tosses. By the above considerations, the probability for tossing head in our thought experiment is a lower bound on the probability that buyer $i$ buys at least one item as long as there are items remaining. As a consequence, the probability for the event of seeing at least $m$ times head is a lower bound on the probability of selling all items in our mechanism.
	
	Using that \[ \Ex[]{Z} = nq = m \log \log n \ ,\] a Chernoff bound with $\delta = 1 - \frac{1}{\log \log n}$ yields
	\begin{align*}
		\Pr{Z < m} &= \Pr{Z < (1 - \delta) \Ex{Z}} \leq \exp\left( - \frac{1}{2} \delta^2 \Ex{Z} \right) \\[0.5em]
		&= \exp\left( - \frac{1}{2} \frac{(\log \log n - 1)^2}{\log \log n} m \right) \stackrel{(1)}{\leq} \exp\left( - \log \log n + 2 \right) = \frac{e^2}{\log n} \,,
	\end{align*}
	where in (1) we assumed that $m \geq 2$. 
	%Observe, that every subadditive buyer will buy at least as many items as a unit-demand buyer. In the latter, buyer $i$ considers buying a remaining item if $v_i(\{j\})$ exceeds the price. Due to our pricing strategy, this occurs with probability $q$. Therefore,  \newline
	
	Combining all these, we can lower-bound the expected social welfare of the posted prices mechanism by 
	\begin{align*}
		\Ex[]{\ALG} & \geq \Ex[]{\revpp} \geq \Pr{\textnormal{all items are sold}} \left(\sum_{j=1}^{m} p_j\right) \geq \Pr{Z \geq m} \sum_{j=1}^{m} F_j^{-1} \left( 1- q \right) \\ & \geq \left( 1 - \frac{e^2}{\log n} \right) \left( 1 - \frac{\log \log \log n + \log m + 1}{\log n} \right) \sum_{j=1}^{m} \Ex[]{\max_{i \in [n]} v_i(\{j\})} \\  & \geq \left( 1 - O \left( \frac{\log\log\log n}{\log n} + \frac{\log m}{\log n}\right) \right) \Ex[]{\OPT} \ .
	\end{align*}	
	
\end{proof}

Observe that the proof of Theorem \ref{theorem:static_mhr_marginals} only requires to bound the expected revenue of our mechanism. Bounding the revenue in the optimal allocation by the expected optimal social welfare, we can state the following corollary.

\begin{corollary}
	The expected revenue achieved by the posted-prices mechanism with subadditive buyers and static prices yields a $1 - O \left( \frac{\log\log\log n}{\log n} + \frac{\log m}{\log n}\right)$-fraction of the expected optimal revenue. 
\end{corollary} 

\subsection{Dynamic Prices}
\label{section:mhr_marginals_dynamic}
In this section, we improve the competitive ratio using dynamic prices instead of static ones. That is, buyer $i$ faces prices depending on the set of available items. Our strategy is to sell specific items only to a subgroup of buyers in order to gain control over the selling process. We can implement this by imposing the following item prices which decrease as the selling process proceeds.

We split the set of buyers in groups of size $\left\lfloor \frac{n}{m} \right\rfloor =: n'$ and sell item $j$ only to the group of buyers \[ \left\{(j-1)\cdot n' + 1,..., (j-1)\cdot n' + n' \right\} =: N_j \enspace . \] For the $k$-th buyer in $N_j$, we set the price for item $j$ to 
\begin{align} \label{prices_dynamic}
	p_j^{((j-1) n' + k)} = F_j^{-1}\left( 1 - \frac{1}{\left\lfloor \frac{n}{m} \right\rfloor - k + 1 } \right)
\end{align} and the prices for all other unsold items to infinity. This choice of prices ensures that the first item is sold among the first $\left\lfloor \frac{n}{m} \right\rfloor$ buyers, the second item among the second $\left\lfloor \frac{n}{m} \right\rfloor$ buyers etc. As a consequence, all items are sold in our process. 

\begin{restatable}{theorem}{dynamicmhrmarginals}
	\label{theorem:dynamic_mhr_marginals}
	The posted-prices mechanism with subadditive buyers and dynamic prices is \newline $1 - O \left( \frac{1 + \log m}{\log n} \right)$-competitive with respect to social welfare. 
\end{restatable}


The proof is deferred to Appendix~\ref{appendix:mhr_marginals}. We mainly use the similar ideas as in the proof for the case with static prices. In the proof of Theorem \ref{theorem:dynamic_mhr_marginals}, we use the revenue as a lower bound for social welfare. Bounding the expected optimal revenue by the expected optimal social welfare, we can state the corollary concerning competitiveness of the revenue.

\begin{corollary}
	The expected revenue of the posted-prices mechanism with subadditive buyers and dynamic prices is a $1 - O \left( \frac{1 + \log m}{\log n}\right)$-fraction of the expected optimal revenue. 
\end{corollary} 

Note that the assumption of buyers' valuations being identically distributed is actually a too strong requirement for these first results. For the proofs in this chapter it would be sufficient to consider buyers having identical marginals on single item sets, but correlations between items might be buyer-specific. 


==> revenue.tex <==
% !TEX root = mhr-prophet.tex
\section{Revenue Considerations}
\label{section:revenue}
In this section, we show how our techniques can also be applied to obtain guarantees on the revenue. To this end, let $\Ex{\revopt}$ be the highest expected revenue among all truthful mechanisms. Clearly $\Ex{\revopt} \leq \Ex{\OPT}$, which will indeed be our benchmark for the positive results.

In this section, we assume that the number of items $m$ is much smaller than the number of buyers $n$. See the respective theorem statements for more details.

\subsection{Static Pricing}
For static pricing, we assume without loss of generality that $m \geq 2$ and set the price of item $j$ to
\[
p_j = \alpha_j F^{-1}(1 - q) \enspace, \text{ where } q = \frac{m \ln \ln n}{n} \enspace.
\]
Note that this effectively means that the ``price per unit'' $\frac{p_j}{\alpha_j} = F^{-1}(1 - q)$ is identical for every item.

\begin{theorem}
The mechanism's expected revenue is at least a $1 - O\left( \frac{\ln \ln \ln n}{\ln n} + \frac{\ln m}{\ln n} \right)$ fraction of the expected optimal welfare (and also revenue).
\end{theorem}

\begin{proof}
By Lemma~\ref{lemma:quantiles1}, we have
\[
F^{-1}(1 - q) \geq \frac{- \ln q}{H_n} \mu_1 = \frac{\ln n - \ln \ln \ln n - \ln m}{H_n} \mu_1 \geq \left( 1 - \frac{\ln \ln \ln n + \ln m + 1}{\ln n} \right) \mu_1 \enspace.
\]

Let $Z$ be the number of buyers of value more than $F^{-1}(1 - q)$. Note that such buyers have a positive utility for every item. So, as long as there are any items remaining, they will buy an item. Therefore, if $Z \geq m$, we are guaranteed that all items are sold. By construction
\[
\Ex{Z} = n q = m \ln \ln n \enspace.
\]
A Chernoff bound with $\delta = 1 - \frac{1}{\ln \ln n}$ yields for the probability that $Z$ is less than $m$
\begin{align*}
	\Pr{Z < m} &= \Pr{Z < (1 - \delta) \Ex{Z}} \leq \exp\left( - \frac{1}{2} \delta^2 \Ex{Z} \right) \\[0.5em]
	&= \exp\left( - \frac{1}{2} \frac{(\ln \ln n - 1)^2}{\ln \ln n} m \right) \stackrel{(1)}{\leq} \exp\left( - \ln \ln n + 2 \right) = \frac{e^2}{\ln n} \,,
\end{align*}

where in (1) we assumed that $m \geq 2$. Therefore, we can lower-bound the expected revenue by
\begin{align*}
	\Ex{\revpp} &\geq \left( \sum_{j = 1}^m p_j \right) \Pr{Z \geq m} \geq \left( 1 - \frac{e^2}{\ln n} \right) \sum_{j = 1}^m \alpha_j F^{-1}(1 - q) \\[0.5em]
	&\geq \sum_{j = 1}^m \alpha_j \left( 1 - \frac{\ln \ln \ln n + \ln m + 1 + e^2}{\ln n} \right) \mu_1 \,.
\end{align*}
Note that $\Ex{\revopt} \leq \Ex{\OPT} \leq \sum_{j = 1}^m \alpha_j \mu_1$. Therefore the claim holds.
\end{proof}

Also this bound is tight for $m \leq \ln \ln n$: By Proposition~\ref{proposition:optimality-static}, for any static price with one item and an exponential distribution, we have
\[
\Ex{\ALG} \leq \left(1 - \Omega\left( \frac{\ln \ln \ln n}{\ln n} \right) \right) \Ex{\OPT} = \left(1 - \Omega\left( \frac{\ln \ln \ln n}{\ln n} \right) \right) H_n \enspace.
\]
Observe that $\Ex{\ALG}$ is clearly an upper-bound on the revenue of the mechanism, whereas the optimal revenue is lower-bounded by the revenue of the second-price auction $\Ex{v_{(2)}} = H_n - 1$. Therefore, this bound also transfers to revenue.

\subsection{Dynamic Pricing}
For dynamic pricing, we set prices in the following way
\[
p_j^{(i)} = \alpha_j F^{-1}\left( 1 - \frac{m}{n - i + 1}\right) \enspace.
\]

\begin{theorem}
The mechanism's expected revenue is at least a $1 - O(\ln m / \ln n)$ fraction of the expected optimal welfare (and also revenue).
\end{theorem}

\begin{proof}
Note that, as the price per unit is identical, buyers will always prefer items with smaller index if they buy any item. Furthermore, the prices are non-increasing. So, we can lower-bound the revenue by assuming that if $v_i \geq F^{-1}\left( 1 - \frac{1}{n - i + 1}\right)$ then the buyer will choose one of the $m$ items uniformly at random and buy it. If it has already been bought, the buyer does not buy anything. 

Let $X_{i, j} = 1$ if buyer $i$ buys the item in this thought experiment. Our goal is to bound
\[
\Ex{\revpp} \geq \Ex{\sum_{i = 1}^{n-m} \sum_{j = 1}^m p^{(i)}_j X_{i, j}} \enspace.
\]
Observe that
\[
\Ex{X_i} = \frac{1}{m} \cdot \frac{m}{n - i + 1} \prod_{i' = 1}^{i - 1} \left( 1 - \frac{1}{m} \cdot \frac{1}{n - i' + 1}\right) = \frac{1}{n} \enspace.
\]
Furthermore,
\[
F^{-1}\left( 1 - \frac{m}{n - i + 1} \right) \geq  \frac{\ln(n - i + 1) - \ln m}{H_n} \mu_1 \enspace.
\]
Therefore
\[
\sum_{i = 1}^{n-m} \sum_{j = 1}^m p^{(i)}_j \Ex{X_i} = \sum_{j = 1}^m \alpha_j \frac{1}{n} \sum_{i = 1}^{n-m} \frac{\ln(n - i + 1) - \ln m}{H_n} \mu_1
\]
Applying that $\sum_{i = 1}^n \ln(n - i + 1) \geq n \ln n - n + (m + 1) - m \ln(m+1)$, this is at least
\[
\sum_{j = 1}^m \alpha_j \frac{\ln n - 1 + \frac{m+1}{n} - \frac{m}{n} \ln(m+1) - \ln m}{H_n} \mu_j \geq \left( 1 - O\left(\frac{\ln m}{\ln n} \right) \right) \sum_{j = 1}^m \alpha_j \mu_j \enspace.
\]
Again we use that $\Ex{\revopt} \leq \Ex{\OPT} \leq \sum_{j = 1}^m \alpha_j \mu_1$.
\end{proof}

Also this bound is optimal.

\begin{proposition}
Even for a single item and an exponential distribution, for every dynamic-price mechanism
\[
\Ex{\revpp} \leq \left( 1 - O\left( \frac{1}{\log n} \right) \right) \Ex{\revopt} \enspace.
\]
\end{proposition}

\begin{proof}
We follow the same approach as in the proof of Proposition~\ref{proposition:optimality-dynamic} but in the space of virtual valuations. We let $v_i \stackrel{\mathrm{i.i.d.}}{\sim} \mathrm{Exp}(1)$. The virtual value function is given by $\phi(t) = t - 1$. The dynamic pricing that maximizes revenue uses the same recursion but on the virtual valuations, having a reserve price of $0$ in the virtual-valuation space. Therefore, it sells to buyer $i$ if $\phi(v_i) \geq r^{(i)}$, where $r^{(n)} = 0$ and $r^{(i)} = \Ex{\max\{r^{(i+1)}, 0, \phi(v_i)\}}$. The expected virtual welfare (and thus revenue) is given by $r^{(0)}$. Consequently, $\Ex{\revpp} \leq r^{(0)}$ for any posted-prices mechanism.

We claim that $r^{(i)} = p^{(i-1)} - 1$, where $p^{(i-1)}$ is as defined in Lemma~\ref{lemma:mdp-recursion}. This follows from a simple induction: We have $r^{(n)} = 0 = 1 - 1 = p^{(n-1)} - 1$. Furthermore, for every $i < n$
\[
r^{(i)} = \Ex{\max\{r^{(i+1)}, 0, \phi(v_i)\}} = \Ex{\max\{p^{(i)} - 1, v_i - 1\}} = \Ex{\max\{p^{(i)}, v_i\}} - 1 = p^{(i-1)} - 1 \enspace.
\]
Consequently, by Lemma~\ref{lemma:mdp-recursion}, we have $r^{(0)} = p^{(-1)} - 1 \leq H_{n+1} - \frac{1}{8} - 1$. For $\Ex{\revopt}$, we use the lower bound $\Ex{\revopt} \geq H_n - 1$ due to the second-price auction.
\end{proof}

==> static.tex <==
% !TEX root = mhr-prophet.tex

\section{Static Pricing}
\label{section:static}
In this section, we consider the problem of using static prices. That is, the price of an item remains unchanged while it is not sold, regardless of how much time has passed or which other items have been sold. We present our first main result, a $1 - O\left(\frac{\log \log \log n}{\log n}\right)$-competitive static-price mechanism as well as a matching impossibility result.

The general design idea for our mechanism is as follows. Given any prices $p_1, \ldots, p_n$, we can consider the probability that a random buyer drawn from the distribution prefers a fixed item. It seems reasonable to adjust prices so that this probability is $\frac{1}{n}$ for every item. This choice would ensure that in expectation one buyer from the sequence will have the item as the first choice. However, in the single-item setting ($\alpha_1 = 1, \alpha_2 = \ldots = 0$), no item except for the first one has any contribution to social welfare and setting the probability to $\frac{1}{n}$ will cause the item not being sold with constant probability. At the same time, there can also be two or more buyers be interested in an item. In the multi-item setting, this has the difficult consequence that when an item is sold buyers will switch to other items instead. That is, the probability of an item being the preferred one increases over time as a consequence of a non-trivial stochastic process. Luckily, we are able to bound the effects in our argument.

In more detail, we define probabilities $q_j$ having the interpretation that a buyer drawn from the distribution has one of items $1, \ldots, j$ as their first choice. For technical reasons, we discard items $m + 1, \ldots, n$ for $m = n - n^{5/6}$ by setting $p_j = \infty$ for these items. For $j \leq m$, we set prices
\[
p_j = \sum_{k = j}^n (\alpha'_k - \alpha'_{k+1}) F^{-1}(1 - q_k) \enspace, \text{ where } q_k = \min\left\{ \frac{k}{n} 2 \ln \ln n, \frac{k}{n} + \sqrt{\frac{\ln n}{n}} \right\} \enspace,
\]
where $\alpha'_k = \alpha_k$ for $k \leq m$ and $0$ otherwise. \later{Maybe there is a more elegant way to deal with this $m$ business.}

Note the similarity of this price definition to the payments when applying the VCG mechanism. There, the buyer being assigned item $j$ has to pay $\sum_{k = j}^n (\alpha'_k - \alpha'_{k+1}) v_{(k + 1)}$.

\begin{theorem}
\label{theorem:staticpositive}
The static-price mechanism is $1 - O\left(\frac{\log \log \log n}{\log n}\right)$-competitive
\end{theorem}

The prices used by the mechanism are fairly low so that we can guarantee that all items are sold with reasonably high probability.

\begin{lemma}
With probability at least $1 - \frac{111}{\ln n}$ all items $1, \ldots, m$ are allocated.
\end{lemma}

\begin{proof}
Let $M^\ast = \{j \mid \alpha'_j > \alpha'_{j+1}\}$ be the set of all items which are strictly better than the following one. Furthermore, let $Z_j$ be the number of buyers of value more than $F^{-1}(1 - q_j)$. If $j \in M^\ast$ and $v_i > F^{-1}(1 - q_j)$, then for all $j' > j$
\[
\alpha'_j v_i - p_j = \alpha'_j v_i - \left( \sum_{k = j}^{j'-1} (\alpha'_k - \alpha'_{k+1}) F^{-1}(1 - q_k) + p_{j'} \right) > \alpha'_j v_i - \sum_{k = j}^{j'-1} (\alpha'_k - \alpha'_{k+1}) v_i - p_{j'} = \alpha'_{j'} v_i - p_{j'} \enspace.
\]
That is, any buyer of value more than $F^{-1}(1 - q_j)$ prefers item $j$ over any item $j+1, \ldots, m$, albeit item $j$ might not be their first choice.

Consider any $j \in M^\ast$. Let $j''$ be the smallest index such that $\alpha'_{j''} = \alpha'_j$ (possibly $j'' = j$). We claim that in the event $Z_j \geq j$, then $\{j'', \ldots, j\}$ are allocated for sure. To see this, we observe that at most $j'' - 1$ buyers can buy one of the items $1, \ldots, j'' - 1$. That is, there are at least $Z_j - (j'' - 1) \geq j - j'' + 1$ buyers who do not buy one of the items $1, \ldots, j'' - 1$ but have value more that $F^{-1}(1 - q_j)$. That is, they prefer every item $j'', \ldots, j$ to any item $j' > j$. Consequently, each of them buys one of the items $j'', \ldots, j$ while they are still available.

Due to this observation, all that remains is to show that with probability at least $1 - \frac{111}{\ln n}$ we have $Z_j \geq j$ for all $j \in M^\ast$.

To this end, we distinguish between two ranges for $j$ and let $j^\ast = \frac{\sqrt{n \ln n}}{2 \ln \ln n - 1}$.

For $j \leq j^\ast$, we have $q_j = \frac{j}{n} 2 \ln \ln n$ and therefore $\Ex{Z_j} = 2 j \ln \ln n$. A Chernoff bound with $\delta = 1 - \frac{2}{\ln \ln n}$ yields for the probability that $Z_j$ is less than $j$
\begin{align*}
	\Pr{Z_j < j} &= \Pr{Z_j < (1 - \delta) \Ex{Z_j}} \leq \exp\left( - \frac{1}{2} \delta^2 \Ex{Z_j} \right) \\[0.5em]
	&= \exp\left( - \frac{(\ln \ln n - 2)^2}{\ln \ln n} j \right) \leq \exp\left( - \left( \ln \ln n - 4 \right) j \right) = \left(\frac{e^4}{\ln n}\right)^j \enspace.
\end{align*}

For $j > j^\ast$, we have $q_j = \frac{j}{n} + \sqrt{\frac{\ln n}{n}}$ and so $\Ex{Z_j} = j + \sqrt{n \ln n}$. Therefore, Hoeffding's inequality gives us
\[
\Pr{Z_j < j} = \Pr{Z_j < \Ex{Z_j} - \sqrt{n \ln n}} \leq \exp\left( - 2 \frac{(\sqrt{n \ln n})^2}{n} \right) = \frac{1}{n^2} \enspace.
\]

In combination, applying the union bound gives us
\[
\Pr{\exists j \in M^\ast: Z_j < j} \leq \sum_{j = 1}^{j^\ast} \left(\frac{e^4}{\ln n}\right)^j + n \frac{1}{n^2} \leq 2 \frac{e^4}{\ln n} + \frac{1}{n} \leq \frac{111}{\ln n} \enspace. \qedhere
\]
\end{proof}

Now, we are ready to prove Theorem~\ref{theorem:staticpositive}.

\begin{proof}[Proof of Theorem~\ref{theorem:staticpositive}]
Our point of comparison will be the VCG mechanism restricted to the first $m$ items. Its expected welfare is
\[
\Ex{\sum_{j = 1}^n \alpha'_j v_{(j)}} \geq \frac{m}{n} \Ex{\sum_{j = 1}^n \alpha_j v_{(j)}} \geq \left( 1 - \frac{1}{n^{1/6}}\right) \Ex{\sum_{j = 1}^n \alpha_j v_{(j)}} \enspace.
\]

To compare the welfare of our mechanism to this VCG welfare, we split it up into the revenue collected by either mechanism and the sum of buyers' utilities. 

\paragraph{Revenue comparison. } With probability $1 - \frac{111}{\ln n}$, all items $1, \ldots, m$ are allocated by our mechanism. Therefore, we can bound the expected revenue
\[
\Ex{\sum_{\text{$j$ is sold}} p_j} \geq \left(1 - \frac{111}{\ln n}\right) \sum_{j = 1}^m p_j = \left(1 - \frac{111}{\ln n}\right) \sum_{j = 1}^m \sum_{k = j}^m (\alpha'_k - \alpha'_{k+1}) F^{-1}(1 - q_k) \enspace.
\]
The expected revenue of VCG is
\[
\Ex{\sum_{j = 1}^m \sum_{k = j}^m (\alpha'_k - \alpha'_{k+1}) v_{(k+1)}} = \sum_{j = 1}^n \sum_{k = j}^n (\alpha'_k - \alpha'_{k+1}) \mu_{k + 1} \enspace.
\]

For $k \leq n^{5/6}$, we use Lemma~\ref{lemma:quantiles1} to get
\begin{align*}
F^{-1}(1 - q_k) & \geq - \frac{\ln(q_k)}{H_n - H_{k-1}} \mu_k \geq \frac{\ln n - \ln(k 2 \ln \ln n)}{H_n - H_{k-1}} \mu_k \geq \frac{\ln n - \ln(k 2 \ln \ln n)}{\ln n - \ln k + 2} \mu_k \\
& \geq \left( 1 - \frac{2 + \ln 2 + \ln \ln \ln n}{\frac{1}{6} \ln n + 2} \right) \mu_k \geq \left( 1 - 20 \frac{\ln \ln \ln n}{\ln n} \right) \mu_k \enspace.
\end{align*}
\later{If this bound really correct?}

For $k > n^{5/6}$, we also use Lemma~\ref{lemma:quantiles1}
\begin{align*}
F^{-1}(1 - q_k) & \geq - \frac{\ln(q_k)}{H_n - H_{k-1}} \mu_k \geq \frac{- \ln\left(\frac{k}{n} + \sqrt{\frac{\ln n}{n}} \right)}{H_n - H_{k-1}} \mu_k \geq \frac{\ln n - \ln(k + \sqrt{n \ln n})}{\ln n - \ln(k-1)} \mu_k
\end{align*}
By concavity of the $\ln$ function, we have $\ln(k + \sqrt{n \ln n}) \leq \ln(k-1) + \frac{1 + \sqrt{n \ln n}}{k - 1}$. So
\[
\frac{\ln n - \ln(k + \sqrt{n \ln n})}{\ln n - \ln (k - 1)} \mu_k \geq \frac{\ln n - \ln(k-1) - \frac{1 + \sqrt{n \ln n}}{k - 1}}{\ln n - \ln(k-1)} \mu_k = \left( 1 - \frac{\frac{1 + \sqrt{n \ln n}}{k - 1}}{\ln n - \ln(k-1)} \right) \mu_k \enspace.
\]
Using $n^{5/6} \leq k - 1 \leq n - n^{5/6}$, we have
\[
(k - 1) \ln\left( \frac{n}{k - 1} \right) \geq n^{5/6} \ln \frac{1}{1 - n^{-1/6}} = n^{2/3} \ln \left( \frac{1}{1 - n^{-1/6}} \right)^{n^{1/6}} \geq n^{2/3}
\]
and therefore, if $n$ is large enough,
\[
\left( 1 - \frac{\frac{1 + \sqrt{n \ln n}}{k - 1}}{\ln n - \ln(k-1)} \right) \mu_k \geq \left( 1 - \frac{1 + \sqrt{n \ln n}}{n^{2/3}} \right) \mu_k \geq \left( 1 - 20 \frac{\ln \ln \ln n}{\ln n} \right) \mu_k \enspace.
\]

By comparing the coefficients, we observe that the revenue of the static price mechanism is within a $1 - O\left(\frac{\ln \ln \ln n}{\ln n}\right)$-factor of the VCG revenue.

\paragraph{Utility comparison. } To compare the buyers' utilities, we exploit that both VCG as well as our static-price mechanism are truthful. Recall that the \emph{virtual value} associated to value $t$ is given by $\phi(t) = t - \frac{1}{h(t)}$. By Myerson's theory \cite{DBLP:journals/mor/Myerson81}, we know that for any truthful mechanism, the expected revenue is equal to the expected virtual welfare. For any truthful mechanism, letting $\textsc{sold}$ denote the set of items that are allocated and, for $j \in \textsc{sold}$, letting $b_j$ be the value of the buyer being allocated the $j$ item, this allows us to rewrite the expected sum of utilities as
\[
\Ex{\sum_{j \in \textsc{sold}} \alpha_j b_j} - \Ex{\sum_{j \in \textsc{sold}} \alpha_j \phi(b_j)} = \Ex{\sum_{j \in \textsc{sold}} \alpha_j \frac{1}{h(b_j)}} \enspace.
\]

We now fix a valuation profile $v$ and compare $\sum_{j \in \textsc{sold}} \alpha_j \frac{1}{h(b_j)}$ between the VCG and the static-price mechanism. By superscripts, we distinguish between the VCG outcome and the static-price outcome (sp). For VCG, we have $b^{\mathrm{VCG}}_j = v_{(j)}$ and $\textsc{sold}^{\mathrm{VCG}} = \{1, \ldots, m\}$. If $\textsc{sold}^{\mathrm{sp}} \supseteq \{1, \ldots, m\}$, we claim that
\[
\sum_{j \in \textsc{sold}^{\mathrm{VCG}}} \alpha'_j \frac{1}{h(b^{\mathrm{VCG}}_j)} \leq \sum_{j \in \textsc{sold}^{\mathrm{sp}}} \alpha'_j \frac{1}{h(b^{\mathrm{sp}}_j)} \enspace.
\]
This is because for all $\ell$ we have
\[
\sum_{j = 1}^\ell \frac{1}{h(b^{\mathrm{VCG}}_j)} = \sum_{j = 1}^\ell \frac{1}{h(v_{(j)})} \leq \sum_{j = 1}^\ell \frac{1}{h(b^{\mathrm{sp}}_j)}
\]
due to the fact that $v_{(1)}, \ldots, v_{(\ell)}$ are the largest $\ell$ entries in $v$ while $b^{\mathrm{sp}}_1, \ldots, b^{\mathrm{sp}}_\ell$ are any $\ell$ entries in $v$ and $\frac{1}{h(\cdot)}$ is non-increasing.
This then combines to
\[
\sum_{j \in \textsc{sold}^{\mathrm{VCG}}} \alpha'_j \frac{1}{h(b^{\mathrm{VCG}}_j)} = \sum_{\ell = 1}^m (\alpha'_\ell - \alpha'_{\ell + 1}) \sum_{j = 1}^\ell \frac{1}{h(b^{\mathrm{VCG}}_j)} \leq \sum_{\ell = 1}^m (\alpha'_\ell - \alpha'_{\ell + 1}) \sum_{j = 1}^\ell \frac{1}{h(b^{\mathrm{sp}}_j)} \leq \sum_{j \in \textsc{sold}^{\mathrm{sp}}} \alpha'_j \frac{1}{h(b^{\mathrm{sp}}_j)} \enspace.
\]

If $\textsc{sold}^{\mathrm{sp}} \not{\supseteq} \{1, \ldots, m\}$, we simply use the fact that the sum of utilities is non-negative. Therefore, we get
\[
\Ex{\sum_{j \in \textsc{sold}^{\mathrm{sp}}} \alpha'_j \frac{1}{H(b^{\mathrm{sp}}_j)}} \geq \left( 1 - \frac{111}{\ln n} \right) \Ex{\sum_{j \in \textsc{sold}^{\mathrm{VCG}}} \alpha'_j \frac{1}{H(b^{\mathrm{VCG}}_j)}} \enspace.
\]
\end{proof}

\subsection{Optimality}
In the following, we will show that the competitive ratio guaranteed by our static-price mechanism in the previous section is indeed optimal. We show that any mechanism using static prices is $1 - \Omega\left(\frac{\ln \ln \ln n}{\ln n}\right)$-competitive. This bound even holds for a single item (so $\alpha_1 = 1$, $\alpha_2 = \ldots = 0$) and the types being drawn from an exponential distribution.

\begin{proposition}
\label{proposition:optimality-static}
	Let $v_1, \dots, v_n \in \mathbb{R}_{\geq 0}$ be random variables where each $v_i$ is drawn i.i.d. from the exponential distribution with rate $1$, i.e., $v_1, \ldots, v_n \sim \mathrm{Exp}(1)$. For all static prices $p \in \mathbb{R}_{\geq 0}$ the competitive ratio of the mechanism picking the first $v_i$ with $v_i \geq p$ is upper bounded by $1 - \Omega\left(\frac{\ln \ln \ln n}{\ln n}\right)$.
\end{proposition}

\begin{proof}
Consider $n \geq e^{e^{e^4}}$.

Observe that always $\Ex{\OPT} = H_n$. Now, we will bound $\Ex{\ALG}$ for any choice of a static price $p \in \mathbb{R}_{\geq 0}$. Regardless of $p$, we have
\[
\Ex{\ALG} = \Ex[]{v \growingmid v \geq p} \cdot \Pr{\exists i: v_i \geq p} = (p + 1) \cdot \left(1 - \left( 1 - e^{-p} \right)^n \right) \enspace.
\]

We will show that for any choice of a static price $p$,
\[
(p + 1) \cdot \left(1 - \left( 1 - e^{-p} \right)^n \right) \leq H_n - c \ln \ln \ln n
\]
for some constant $c$, which then immediately proves the claim as $H_n = \Theta(\ln n)$.

To this end, we will consider three cases for the choice of $p$.

\paragraph{Case 1: } $0 \leq p < \ln n - \frac{1}{2} \ln \ln \ln n$: We use the trivial upper bound of $1$ for the probability term in $\Ex{\ALG}$, so
		\begin{align*}
		(p + 1) \cdot \left(1 - \left( 1 - e^{-p} \right)^n \right) & \leq (p + 1)  < \ln n - \frac{1}{2} \ln \ln \ln n + 1 \\
		& \leq \ln n - \frac{1}{2} \ln \ln \ln n + \frac{1}{4} \ln \ln \ln n = \ln n - \frac{1}{4} \ln \ln \ln n
		\end{align*}
		as $n \geq e^{e^{e^4}}$ holds.
		
\paragraph{Case 2: } $\ln n - \frac{1}{2} \ln \ln \ln n \leq p \leq H_n - 1$: Again, observe that the expected value of the algorithm can be upper bounded by
		\begin{align*}
		&(p + 1) \cdot \left(1 - \left( 1 - e^{-p} \right)^n \right) \leq H_n \cdot \left(1 - \left( 1 - e^{-p} \right)^n \right) \\
		&\leq H_n \cdot \left(1 - \left( 1 - e^{-\ln n + \frac{1}{2} \ln \ln \ln n} \right)^n \right) = H_n \cdot \left(1 - \left( 1 - \frac{\sqrt{\ln \ln n}}{n} \right)^n \right) \,.
		\end{align*}
		
		Next, we want to lower bound $\left( 1 - \frac{\sqrt{\ln \ln n}}{n} \right)^n$ in order to get the desired upper bound on $\Ex[]{\textnormal{ALG}}$. For this purpose, we use the following inequality.
		
%\begin{lemma}[\todo{reference}]
%	\label{lemma:lower_bound_on_oneplusxovern}
	For $n > 1$ and $x \in \mathbb{R}$ with $\lvert x\rvert \leq n$, we have
	\begin{align*}
	\left( 1 + \frac{x}{n} \right)^n \geq e^x \cdot \left( 1 - \frac{x^2}{n} \right) \,.
	\end{align*}
%\end{lemma}
\later{Reference?}

This way, we get
		\begin{align*}
		\left( 1 - \frac{\sqrt{\ln \ln n}}{n} \right)^n &\geq e^{-\sqrt{\ln \ln n}} \cdot \left( 1 - \frac{(- \sqrt{\ln \ln n})^2}{n} \right) = e^{-\sqrt{\ln \ln n}} \cdot \underbrace{\left( 1 - \frac{\ln \ln n}{n} \right)}_{\geq \frac{1}{2} ,\;\forall n} \geq \frac{1}{2} e^{-\sqrt{\ln \ln n}} \,.
		\end{align*}
		
		Note that if $\ln \ln n \geq 4$, then also $\sqrt{\ln \ln n} \leq \frac{1}{2} \ln \ln n$ and therefore 
		\[
		e^{-\sqrt{\ln \ln n}} \geq e^{- \frac{1}{2} \ln \ln n} = \frac{1}{\sqrt{\ln n}} \enspace.
		\]
		
		This gives us
		\begin{align*}
		(p + 1) \cdot \left(1 - \left( 1 - e^{-p} \right)^n \right) &\leq H_n \cdot \left(1 - \left( 1 - \frac{\sqrt{\ln \ln n}}{n} \right)^n \right) \leq H_n \cdot \left( 1 - \frac{1}{2} e^{-\sqrt{\ln \ln n}} \right) \\
		&\leq H_n \cdot \left( 1 - \frac{1}{2\sqrt{\ln n}} \right) \leq H_n \cdot \left( 1 - \frac{\ln \ln \ln n}{2 \ln n} \right) \enspace,
		\end{align*}
		where in the last step we use that $\sqrt{\ln n} \geq \ln \ln \ln n$ and therefore $\sqrt{\ln n} \leq \frac{\ln n}{\ln \ln \ln n}$.
		
\paragraph{Case 3: } $p > H_n - 1$: In this case we use the fact that Giannakopoulos and Zhu \cite{DBLP:conf/wine/GiannakopoulosZ18} showed that the revenue function $p \mapsto p \cdot \left(1 - \left( 1 - e^{-p} \right)^n\right)$ is non-increasing on $[H_n - 1, \infty)$. 

We can conclude that
		\begin{align*}
		 (p + 1) \cdot \left(1 - \left( 1 - e^{-p} \right)^n \right) & \leq p \cdot \left(1 - \left( 1 - e^{-p} \right)^n \right)+ 1 \leq H_n \cdot \left(1 - \left( 1 - e^{-(H_n - 1)} \right)^n \right)+ 1 \\
		&\leq H_n \cdot \left(1 - \left( 1 - \frac{e}{n} \right)^n \right)+ 1 \leq \frac{99}{100} H_n + 1
		\end{align*}
\end{proof}
